Prototypes are Balanced Units for Efficient and Effective Partially Relevant Video Retrieval

In a retrieval system, simultaneously achieving search accuracy and efficiency is inherently challenging. This challenge is particularly pronounced in partially relevant video retrieval (PRVR), where incorporating more diverse context representations at varying temporal scales for each video enhances accuracy but increases computational and memory costs. To address this dichotomy, we propose a prototypical PRVR framework that encodes diverse contexts within a video into a fixed number of prototypes. We then introduce several strategies to enhance text association and video understanding within the prototypes, along with an orthogonal objective to ensure that the prototypes capture a diverse range of content. To keep the prototypes searchable via text queries while accurately encoding video contexts, we implement cross- and uni-modal reconstruction tasks. The cross-modal reconstruction task aligns the prototypes with textual features within a shared space, while the uni-modal reconstruction task preserves all video contexts during encoding. Additionally, we employ a video mixing technique to provide weak guidance to further align prototypes and associated textual representations. Extensive evaluations on TVR, ActivityNet-Captions, and QVHighlights validate the effectiveness of our approach without sacrificing efficiency.

==> tabs/tab2_anet.tex <==
\begingroup
\setlength{\tabcolsep}{1.9pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.} % Default value: 1
\begin{table}[t]
\centering
 \footnotesize
{
 \caption{Performances on ActivityNet Captions. $\dagger$ indicates the usage of different splits with currently unavailable videos.}
 \label{table_anet}
 \begin{tabular}{lccccccc}
 \hlineB{2.5}
 Model  & R@1 & R@5 & R@10 & R@100 & SumR & Memory~(MB) \\ \hlineB{2.5}
\multicolumn{7}{c}{I3D + Roberta} \\ \hlineB{2.5}
\multicolumn{7}{l}{\textit{VCMR methods without moment localization}} \\ 
 % W2VV& 2.2 & 9.5 & 16.6 & 45.5  & 73.8 & - \\
 % HTM & 3.7 & 13.7& 22.3 & 66.2  & 105.9 & - \\
 % HGR & 4.0& 15.0  & 24.8 & 63.2  & 107.0 & - \\
 % RIVRL & 5.2 & 18.0  & 28.2 & 66.4  & 117.8& - \\
 % DE++& 5.3 & 18.4& 29.2 & 68.0 & 121.0 & - \\
 % CE& 5.5 & 19.1& 29.9 & 71.1  & 125.6 & - \\
 % CLIP4Clip& 5.9 & 19.3& 30.4 & 71.6  & 127.3 & - \\
 % Cap4Video& 6.3 & 20.4& 30.9 & 72.6  & 130.2 & - \\
 ReLoCLNet& 5.7 & 18.9& 30.0& 72.0 & 126.6 & - \\
 XML & 5.3 & 19.4& 30.6 & 73.1  & 128.4 & - \\
 CONQUER& 6.5 & 20.4& 31.8 & 74.3  & 133.1 & - \\ \hline
 MS-SL  & 7.1 & 22.5& 34.7 & 75.8  & 140.1 & 0.98 \\
 % ((481397 / 4430) + 528 ) * 384 * 4 = 977921
 GMMFormer& 8.3 & 24.9& 36.7 & 76.1  & 146.0& 0.05 \\
 \rowcolor{gray!30}
 Ours& 7.5 & 25.2 & 37.4 & 77.3 & \textbf{147.5} & 0.09 \\ \hlineB{2.5}
 \multicolumn{7}{c}{I3D + Roberta + CLIP B/32} \\ \hlineB{2.5}
 DL-DKD & 8.0& 25.0 & 37.4 &77.1  & 147.6 & 0.39 \\ \hlineB{2.5}
 \multicolumn{7}{c}{CLIP L/14} \\ \hlineB{2.5}
 % 120910 (super image 2x2기준 각 비디오마다 4로나눠서 올림) / 4430 * 768 * 4 = 98,132.0018
 % 0.5 fps : 13974
 % QASIR 2x2$\dagger$&  18.2 & 39.6 & 52.2 & 84.8  & 194.9& 0.14 \\ \hline
 MS-SL  & 14.9 & 37.9 & 51.4 & 85.2 & 189.4 & 0.99 \\
 % 525333 frames / 4430 (val data) = 118.585 + 528
% * 384 * 4B = 993155.0627 B = 
 GMMFormer & 15.5 & 37.9 & 51.0 & 84.2 & 188.6 & 0.05 \\
 \rowcolor{gray!30}
 Ours & 15.4 & 38.8 & 52.3 & 85.2 & \textbf{191.6} & 0.09 \\ \hlineB{2.5}
 
 % \rowcolor{gray!30}
 % Ours$\dagger$ & & & & & & 0.09 \\ \hline
 % \hlineB{2.5}
 \end{tabular}
}
\end{table}
\endgroup


% \begingroup
% \setlength{\tabcolsep}{6pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.} % Default value: 1
% \begin{table}[t]
% {
%  \centering
%  \small
%  \caption{Performances on ActivityNet Captions. $\dagger$ indicates the usage of different splits.}
%  \label{table_anet}
%  \begin{tabular}{l|ccccc|cc}
%  \hlineB{2.5}
%  Model  & R@1 & R@5 & R@10 & R@100 & SumR & Mem.~(MB) & Time~(s) \\ \hline
% \multicolumn{7}{c}{ResNet152 + I3D + Roberta} \\ \hline
%  W2VV& 2.2 & 9.5 & 16.6 & 45.5  & 73.8 & -&-  \\
%  HTM & 3.7 & 13.7& 22.3 & 66.2  & 105.9 & -&-  \\
%  HGR & 4& 15  & 24.8 & 63.2  & 107 & -&-  \\
%  RIVRL & 5.2 & 18  & 28.2 & 66.4  & 117.8& -&-  \\
%  DE++& 5.3 & 18.4& 29.2 & 68 & 121 & -&-  \\
%  CE& 5.5 & 19.1& 29.9 & 71.1  & 125.6 & -&-  \\
%  CLIP4Clip& 5.9 & 19.3& 30.4 & 71.6  & 127.3 & -&-  \\
%  Cap4Video& 6.3 & 20.4& 30.9 & 72.6  & 130.2 & -&- \\
%  ReLoCLNet& 5.7 & 18.9& 30& 72 & 126.6 & -&- \\
%  XML & 5.3 & 19.4& 30.6 & 73.1  & 128.4 & -&- \\
%  CONQUER& 6.5 & 20.4& 31.8 & 74.3  & 133.1 & -&- \\
%  MS-SL  & 7.1 & 22.5& 34.7 & 75.8  & 140.1 & 0.98MB& - \\
%  % ((481397 / 4430) + 528 ) * 384 * 4 = 977921
%  GMMFormer& 8.3 & 24.9& 36.7 & 76.1  & 146& 0.05MB & - \\
%  \rowcolor{gray!30}
%  Ours& 7.7 & 25.1 & 37.5 & 77.3 & 147.6 & 0.09MB &-\\ \hline
%  \multicolumn{7}{c}{ResNet152 + I3D + Roberta + CLIP B/32} \\ \hline
%  DL-DKD & 8.0& 25.0 & 37.4 &77.1  & 147.6 & - &-\\ \hline
%  \multicolumn{7}{c}{CLIP L/14} \\ \hline
%  % 120910 (super image 2x2기준 각 비디오마다 4로나눠서 올림) / 4430 * 768 * 4 = 98,132.0018
%  % 0.5 fps : 13974
%  MS-SL  & 14.9 & 37.9 & 51.4 & 85.2 & 189.4 & 0.99MB &-\\
%  % 525333 frames / 4430 (val data) = 118.585 + 528
% % * 384 * 4B = 993155.0627 B = 
%  GMMFormer & 15.5 & 37.9 & 51 & 84.2 & 188.6 & 0.05MB & -\\
%  \rowcolor{gray!30}
%  Ours & & & & & 193 & 0.09MB & - \\ \hline
%  QASIR 2x2$\dagger$&  18.2 & 39.6 & 52.2 & 84.8  & 194.9& 0.14MB & - \\
%  \rowcolor{gray!30}
%  Ours$\dagger$ & & & & & & 0.09MB & -\\ \hline
%  \hlineB{2.5}
%  \end{tabular}
% }
% \end{table}
% \endgroup



==> tabs/tab3_cha.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begingroup
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.} % Default value: 1
\begin{table}
\centering
 \small
{
 \caption{Performances on Charades Captions.}
 \label{table_charades}
 \begin{tabular}{l|ccccc|cc}
 \hlineB{2.5}
 Model & R@1 & R@5 & R@10 & R@100 & SumR & Mem.~(MB) & Time~(s) \\ \hline
 \multicolumn{8}{c}{ResNet152 + I3D + Roberta} \\  \hline
 W2VV& 0.5& 2.9& 4.7 & 24.5 & 32.6& -& -\\
 HGR & 1.2& 3.8& 7.3 & 33.4 & 45.7&  & -\\
 CE  & 1.3& 4.5& 7.3 & 36& 49.1&  & -\\
 DE++& 1.7& 5.6& 9.6 & 37.1 & 54.1&  & -\\
 RIVRL & 1.6& 5.6& 9.4 & 37.7 & 54.3&  & -\\
 HTM & 1.2& 5.4& 9.2 & 44.2 & 60  &  & -\\
 CLIP4Clip & 1.8& 6.5& 10.9& 44.2 & 63.4& & - \\
 Cap4Video & 1.9& 6.7& 11.3& 45& 65  &  & -\\
 ReLoCLNet & 1.2& 5.4& 10  & 45.6 & 62.3&  & -\\
 XML & 1.6& 6  & 10.1& 46.9 & 64.6&  & -\\
 CONQUER & 1.8& 6.3& 10.3& 47.5 & 66  &  & -\\
 MS-SL & 1.8& 7.1& 11.8& 47.7 & 68.4&  & -\\
 PEAN& 2.7& 8.1& 13.5& 50.3 & 74.7&  & -\\
 GMMFormer & 2.1& 7.8& 12.5& 50.6 & 72.9& & - \\ 
 \rowcolor{gray!30}
 Ours& - & - & - & - & - & - & - \\ \hlineB{2.5}
 \multicolumn{8}{c}{CLIP L/14} \\ \hline
 MS-SL &  & & &  & & 0.14MB \\
 % 117608 / 1334 * 384 * 4 = 135,416.7076461769
 GMMFormer & & & & & & 0.05MB \\ 
 \rowcolor{gray!30}
 Ours & - & - & - & - & - &  0.09MB & - \\ \hlineB{2.5}
 \end{tabular}
}
\end{table}
\endgroup


==> tabs/tab_uniablation.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begingroup
\setlength{\tabcolsep}{1.0pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.94} % Default value: 1
\begin{table}[t]
\centering
{
 \small
 \caption{
 % Design ablation for uni-modal reconstruction on TVR with CLIP/L-14 backbone. 
 % U.task indicates whether mask or na\"ive reconstruction is employed.
 % U.Dec and C.Dec denote the decoder architecture for uni- and cross-modal reconstruction where T and M denote transformer-based and MLP-based decoders, respectively. 
 % Note that T+M stands for the decoder consisting of both self-attention and MLP layers. 
 Ablation study on uni-modal reconstruction.% for the TVR dataset using the CLIP/L-14 backbone. 
 `Cross.' column indicates whether cross-modal mask reconstruction is used. 
 `U.task' and `U.Dec.' refer to the uni-modal reconstruction task type and decoder architecture, respectively. 
 `T' and `M' denote transformer- and MLP-based decoders, while `T+M' represents a combined decoder. % decoder combining self-attention and MLP. 
 Results for each design solely are in (ii), (iv), and (vi) while compatibility with the cross-modal reconstruction is shown in (iii), (v), and (vii).
 % 'Cross.' column indicates whether the cross-modal mask reconstruction is employed or not.
 % 'U.task' and 'U.Dec' refer to the type of reconstruction task and the decoder architecture for the uni-modal scenario, respectively.  
 % 'T' and 'M' denote transformer-based and MLP-based decoders, and 'T+M' indicates a decoder that integrates self-attention and MLP layers.
 % We report the results when each design is solely applied in (ii), (iv), and (vi) while (iii), (v), and (vii) shows the compatibility with the cross-modal reconstruction task.
 % However, it is important to note that designs using a transformer in the decoder are incompatible with the cross-modal mask reconstruction task, as shown in rows (iii) and (v). 
 }
 \label{table_unimodal_ablation}
 \begin{tabular}{c|c|cc|ccccc}
 \hlineB{2.5}
 & Cross. & \multicolumn{1}{c}{U.task} & \multicolumn{1}{c|}{U.Dec.} & R@1 & R@5 & R@10 & R@100 & SumR \\ \hline
 % - & - & - & 32.8 & 58.2 & 68.6 & 93.4 & 253.0 \\ \hline
 \rowcolor{gray!20}
 i & \checkmark & \xmark & \xmark & 32.9 & 58.7 & 69.0 & 93.5 & 254.2$_{(
 \pm0.0)}$ \\ \hline
 ii & \xmark & mask & T &  32.9 & 58.8 & 68.9 & 93.6 & 254.2 \\ 
 iii & \checkmark & mask & T & 32.8 & 57.9 & 68.5 & 94.9 & 253.1$_{(-1.1)}$ \\ \hline
 iv & \xmark & recon & T+M & 33.0 & 58.5 & 68.3 & 93.8 & 253.3 \\ 
 v & \checkmark &recon & T+M & 32.8 & 58.5 & 68.7 & 94.0 & 254.0$_{(-0.2)}$ \\ \hline
 vi & \xmark & recon & M &  32.9 & 58.1 & 68.4 & 93.4 & 252.7 \\ 
 vii & \checkmark & recon & M & 33.8 & 58.7 & 68.8 & 93.9 & 255.1$_{(+0.9)}$ \\ 
 \hlineB{2.5}
 \end{tabular}
}
\end{table}
\endgroup

